Control-Oriented System Identification: Classical, Learning, and Physics-Informed Approaches

We survey classical, machine learning, and data-driven system identification approaches to learn control-relevant and physics-informed models of dynamical systems. Recently, machine learning approaches have enabled system identification from noisy, high-dimensional, and complex data. However, their utility is limited by their ability to provide provable guarantees on control-relevant properties. Meanwhile, control theory has identified several properties that are useful in analysis and control synthesis, such as dissipativity, monotonicity, energy conservation, and symmetry-preserving structures. We posit that merging system identification with such control-relevant or physics-informed properties can provide useful inductive bias, enhance explainability, enable control synthesis with provable guarantees, and improve sample complexity. We formulate system identification as an optimization problem where control-relevant properties can be enforced through direct parameterization (constraining the model structure to satisfy a desired property by construction), soft constraints (encouraging control-relevant properties through regularization or penalty terms), and hard constraints (imposing control-relevant properties as constraints in the optimization problem). Through this lens, we survey methods to learn physics-informed and control-relevant models spanning classical linear and nonlinear system identification, machine learning approaches, and direct identification through data-driven and behavioral representations. We also provide several expository examples that are accompanied by code and brief tutorials on a public Github repository. We also describe challenging directions for future research, including identification in networked, switched, and time-varying systems, experiment design, and bridging the gaps between data-driven, learning-based, and control-oriented approaches.

==> tex/Section4_backup_detailedversion.tex <==
\textit{Modeling system dynamics with physics-informed neural networks based on Lagrangian mechanics} (\cite{roehrl2020modeling}). 

Considers the Lagrangian dynamics of the form, 
\begin{equation}
\label{eq:}
    f^{-1}(q,\dot{q}, \ddot{q}) = M(q)\ddot{q} + C(q,\dot{q})\dot{q} + G(q) = \tau\,,
\end{equation}
where $M(q)$ is the inertia matrix, $C(q,\dot{q})$ is the Coriolis matrix and $G(q)$ is the conservative forces, e.g. gravity, and $\tau$ is the non-conservative forces, approximated by a neural network $\tau(q, \dot{q}, u;\theta)$ with input $q, \dot{q}$, control input $u$ and parameter $\theta$. Given a dataset of the form $\mathcal{D} = \{q_i, \dot{q}_i\}_{i=1}^N$, the paper uses one step of 4th order Runge-Kutta method to integrate the dynamics and predict the states $\hat{\mathcal{D}} = \{\hat{q}_i, \dot{\hat{q}}_i\}_{i=1}^N$. The discrepancy between $\mathcal{D}$ and $\hat{\mathcal{D}}$ is used to train the neural network $Q$, by backpropagating through the Runge-Kutta step. This is different from Neural ODE where the backprogpagation is done using adjoint method and the common solver is Runge-Kutta 45 method (with adaptive step size), leading to better accuracy. Even though the control input is included in the model, the paper did not design a controller for the learned system.

\textit{Deep Lagrangian Networks: Using Physics as Model Prior for Deep Learning (DeLAN)} \cite{lutter2019deeplagrangian}: This paper instead models $M(q) = L(q)L(q)^\top$ and $G(q)$ as neural networks with parameter $\theta$ and describes $C(q,\dot{q}$ in terms of $L(q)$. The approximated inverse dynamics $\hat{f}^{-1}(q,\dot{q}, \ddot{q};\theta)$ is compared with $\tau$ from the dataset to train the model. This approach avoids the need of an ODE solver but requires $\ddot{q}$ in the dataet. No controller was derived either.

\textit{A General Framework for Structured Learning of Mechanical Systems} \cite{gupta2019general}. This paper also considers the inverse dynamics $f^{-1}(q,\dot{q}, \ddot{q}) = \tau$ above but learn $M(q) = L(q)L(q)^\top$, $G(q)$ and $\tau(q, \dot{q}, u)$ from data. The training is done through one Runge-Kutta step like \cite{roehrl2020modeling}. The learned model is then used to plan a trajectory using Direct Collocation trajectory Optimization (DIRCOL) and design a time-varying linear quadratic regulator (TVLQR) controller to track the trajectory.

\textit{Lagrangian neural networks} \cite{cranmer2020lagrangian}. This paper is similar to \cite{lutter2019deeplagrangian} but consider a general Lagrangian dynamics instead of one for rigid-body dynamics. Therefore, it can be applied to other systems, e.g. in physics, rather than robotics. The paper also illustrates that the Lagrangian neural networks can handle systems with disconnected coordinates such as graphs.

\textit{Deep Lagrangian Networks for end-to-end learning of energy-based
control for under-actuated system}~\cite{lutter2019deepunderactuated}. This paper extends \cite{lutter2019deeplagrangian} by modeling the Hamiltonian of the system and shows that the total energy of the learned system is conserved. It also designs energy-based controller for a class of simple under-actuated systems such as Furuta pendulums, cartpoles and acrobots.


\textit{Hamiltonian neural networks} \cite{greydanus2019hamiltonian}. This paper considers learning Hamiltonian formulation of a system instead of Lagrangian dynamics. Let $q \in \mathbb{R}^n$ and $p\in \mathbb{R}^n$ be the generalized coordinates and momentum of a system, respectively. The Hamiltonian dynamics on $\mathbb{R}^n$ are described as:
\begin{equation} \label{eq:hamiltonian_dynamics_Rn}
    \frac{dq}{dt} = \frac{\partial H}{\partial p}, \frac{dp}{dt} = -\frac{\partial H}{\partial q}, 
\end{equation}
where $H$ denotes the total energy of the system. The Hamilton's equations of motion \eqref{eq:hamiltonian_dynamics_Rn} guarantees that $\frac{dH}{dt} =0$, i.e. the total energy is conversed along the trajectory. To learn an unknown dynamics, the total energy $H$ is modeled as a neural network with parameter $\theta$. The training loss describe the deviation from the Hamilton's equations as follows.
\begin{equation}
    \mathcal{L}_{HNN} = \left\Vert \frac{dq}{dt} - \frac{\partial H}{\partial p} \right\Vert_2 + \left\Vert \frac{dp}{dt} +\frac{\partial H}{\partial q} \right\Vert_2.
\end{equation}
Similar to many Lagrangian-based models above, this approach requires availability of the derivative of the momentum, i.e. availability of the second-order derivation of the coordinates $q$. No control design was proposed for the learned system.

\textit{On Learning Hamiltonian Systems from Data} \cite{bertalan2019learning}. This paper considers the Hamiltonian dynamics on $\mathbb{R}^n$ as shown in \eqref{eq:hamiltonian_dynamics_Rn} but with observations of the coordinates $q$ and momentum $p$, e.g. images. The Hamilton's dynamics are modeled using Gaussian process or a neural network on a latent space of the coordinates and momentum, learned from the observations using an auto-encoder. The auto-encoder and the Hamiltonian dynamics model are trained simultaneously in an end-to-end manner. No control design was proposed.

\textit{Symplectic recurrent neural networks} \cite{chen2019symplectic}. This paper gets rid of the need to have the second-order derivatives of the coordinates $q$ in the dataset by using a leapfrog integrator. The loss, describing the discrepancy between the predictions and ground-truth values of the coordinates and momentum, is backpropagated using the explicit update steps in the integrator, equivalent to backpropagating through time in recurrent neural networks.

\textit{Symplectic ODE-Net: learning Hamiltonian dynamics with control} \cite{zhong2020symplectic}. Instead of using a leapfrog integrator with explicit update rules  \cite{chen2019symplectic}, this paper uses neural ODE \cite{chen2018neural} with Hamiltonian structure to approximate the unknown dynamics. The loss is back-propagated using adjoint method, eliminating the needs to have second-order derivative of the coordinates $q$. An energy-shaping regulation controller is designed for fully-actuated systems.

\textit{Simplifying Hamiltonian and Lagrangian Neural
Networks via Explicit Constraints} \cite{finzi2020simplifying}. Finzi et al. show that it is better, in terms of accuracy and data efficiency, to learn Lagrangian and Hamiltonian dynamics with Cartesian coordinates with explicit manifold constraints instead of generalized coordinates. Constraint violations are penalized by using Lagrange multipliers.

\textit{Hamiltonian-based neural ode networks on the $SE(3)$ manifold for dynamics learning and control} \cite{duong2021hamiltonian}. This paper considers learning Hamiltonian dynamics on $SE(3)$ manifold, that encodes Hamiltonian dynamics and the $SE(3)$ manifold constraints on the architecture of a neural ODE network. This is suitable for learning the dynamics of single-rigid-body robots such as ground vehicles and UAV, where the orientation is often described by a rotation matrix on the $SO(3)$ manifold. An energy-based controller is designed for trajectory tracking tasks for both fully and under-actuated systems such as quadrotors.

\textit{Port-Hamiltonian neural networks in multi-agent settings} \cite{furieri2022distributed, sebastian2022lemurs}.
    % \textit{Distributed neural network control with dependability guarantees: a compositional port-Hamiltonian approach} \cite{furieri2022distributed}. 
\cite{furieri2022distributed} designs a distributed deep neural network control policies with stability guarantees for port-Hamiltonian systems. The dynamic controller is modeled as another port-Hamiltonian system, whose output is the control input for the original systems. The controller parameters are trained to minimize a pre-defined cost function for the task.
    % \textit{LEMURS: Learning Distributed Multi-Robot Interactions} \cite{sebastian2022lemurs}. 
\cite{sebastian2022lemurs} learns a control policy from demonstrations for port-Hamiltonian dynamics. The control policy is derived using the interconnection and damping assignment passivity-based control (IDA-PBC) approach, where the robots interact by exchanging or dissipating energy based on the state of their neighbors. The energy exchange and dissipation are then modeled as neural networks with self-attention architecture to handle time-varying topology and offer scalability.

\textit{Port-Hamiltonian neural networks in multi-agent settings \todo{YY's comment: move this part to a different place?}} \cite{furieri2022distributed, sebastian2022lemurs}.

\cite{furieri2022distributed} designs a distributed deep neural network control policies with stability guarantees for port-Hamiltonian systems. The dynamic controller is modeled as another port-Hamiltonian system, whose output is the control input for the original systems. The controller parameters are trained to minimize a pre-defined cost function for the task.
    % \textit{LEMURS: Learning Distributed Multi-Robot Interactions} \cite{sebastian2022lemurs}. 
\cite{sebastian2022lemurs} learns a control policy from demonstrations for port-Hamiltonian dynamics. The control policy is derived using the interconnection and damping assignment passivity-based control (IDA-PBC) approach, where the robots interact by exchanging or dissipating energy based on the state of their neighbors. The energy exchange and dissipation are then modeled as neural networks with self-attention architecture to handle time-varying topology and offer scalability.

\JF{\cite{pfrommer2021contactnets} proposes Contactnets to model the discontinuous contact dynamics for robot manipulation tasks. Instead of directly learning the contact forces, this model learns the inter-body distance $d(q)$ and the contact-frame normal impulses $\lambda$, where $q$ depicts the robot configuration and object poses. Considering rigid bodies, contact behaviors have two essential behaviors: normal forces push bodies apart when they touch; normal forces should be chosen to maximize the mechanical power loss during contact. To incorporate the prior knowledge and the assumption for rigid bodies, three soft penalty terms are introduced: 1) non-zero force without contact; 2) negative inter-body distance induced by the estimated, i.e. motion generated by the forces should not cause penetration; 3) maximize the power loss. This model is based on analytical contact dynamics for inelastic collision with rigid objects, elastic effects are not considered. No controllers are derived. }

\JF{\cite{skomski2021constrained} presents constrained block nonlinear neural state space models to learn nonlinear dynamical systems, where different blocks are applied based on the interactions of the components of the nonlinear system. Specifically, when the input $u_t$ and the current state $x_t$ are disentangled, the next state can be predicted with two neural networks $x_{t+1}=f_{\theta_1}(x_t)+f_{\theta_2}(u_t)$ instead of using one neural network. In this case, two components can incorporate different priors. The constraints considered in the paper include output constraints (with lower and upper bounds), input sensitivity, and state smoothing, where state smoothing means minimizing the difference between two consecutive states. All constraints are enforced as soft penalties punishing the violations.}

\JF{\cite{lechner2020gershgorin} proposes to model the hidden states evolution as a linear dynamical system, i.e. $\dot{x}=Ax+Bu$, where $u$ is the input, $x$ is the hidden state, $A,\,B$ are learnable parameters. The algorithm is applied to imitation learning for robots to mimic demonstrations. To achieve stable internal state updates, the eigenvalues of the $A$ should have negative real parts. The Gershgorin circle loss is introduced to enforce the negativity of eigenvalues of $A$. Specifically, the loss is written as follows,
$$\mathcal{L}=\sum_{i=1}^n\max\{0,A_{i,i}+\sum_{j\neq i}|A_{i,j}|+\epsilon\},\ \epsilon>0$$
Following the Gershgorin circle theorem, every eigenvalue of $A$ lies within at least one of the Gershgorin discs $D(A_{i,i},R_i)$, where $R_i=\sum_{j\neq i}|A_{i,j}|$ and $D(a,b):=\{x\in\mathbb{C}\big | \lvert x-a\rvert\leq b\}$. Thus when the loss $\mathcal{L}\leq 0$ then all eigenvalues of $A$ have a negative real part. The algorithm is applied for imitation learning so it is the controller. }

\JF{\cite{schlaginhaufen2021learning} aims to learn stable deep dynamics models with partial observations. Because of the partial observability, the ODE system is not Markovian anymore, i.e. the temporal transition is not uniquely dependent on the current state. To model the non-Markovian effect, this work incorporates the neural delay differential equations (NDDEs) from \cite{zhu2021neural}to include previous states instead of estimating the non-observed data. Thus the model can be represented as a time-delay system. To guarantee stability, the Lyapunov-Razumikhin function \cite{jankovic2001control} is applied to guarantee stability for the time-delay system. The Lyapunov-Razumikhin function shares the same structure as a standard Lyapunov function but with a stronger stability condition to compensate for the time delay. As a result, the same neural Lyapunov function from \cite{kolter2019learning} is adopted, and the Lyapunov-Razumikhin conditions are penalized with a soft penalty. If the penalty is zero along the trajectories, the learned NDDEs are stable. }
